Hardware Scaling Trends and Diminishing Returns in Large-Scale Distributed Training

Dramatic increases in the capabilities of neural network models in recent years are driven by scaling model size, training data, and corresponding computational resources. To develop the exceedingly large networks required in modern applications, such as large language models (LLMs), model training is distributed across tens of thousands of hardware accelerators (e.g. GPUs), requiring orchestration of computation and communication across large computing clusters. In this work, we demonstrate that careful consideration of hardware configuration and parallelization strategy is critical for effective (i.e. compute- and cost-efficient) scaling of model size, training data, and total computation. We conduct an extensive empirical study of the performance of large-scale LLM training workloads across model size, hardware configurations, and distributed parallelization strategies. We demonstrate that: (1) beyond certain scales, overhead incurred from certain distributed communication strategies leads parallelization strategies previously thought to be sub-optimal in fact become preferable; and (2) scaling the total number of accelerators for large model training quickly yields diminishing returns even when hardware and parallelization strategies are properly optimized, implying poor marginal performance per additional unit of power or GPU-hour.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/0_outline.tex <==
\section{Methodology}

\subsection{System Components}
What are limiting factors for components ? 
\begin{enumerate}
    \item Hardware Accelerator
    \begin{enumerate}
        \item  Warps executing waves of thread blocks for kernel arithmetic operations on SM cores at the target precision
        \item Limiting Component: Computation; HBM VRAM Access; CPU-GPU Host Operations (Activation Checkpointing and Offloading)
    \end{enumerate}
    \item Multiple GPUs on an Individual Node
    \begin{enumerate}
        \item Limiting Component: Computation; NVLink or PCIe communication
    \end{enumerate}
    \item Individual Nodes Connected via a Single Switch: NVLink communication
    \item Individual Nodes Contained on a Single Rail: Network Fabric (Infiniband, EFA)
    \item Multiple Connected Rails: Network with additional director switch overhead
\end{enumerate}

\subsection{Performance Metrics }
\begin{itemize}
    \item Tokens per GPU per second
    \item  Latency per global batch of size K
    \item  Hardware and Model FLOPs Utilization
    \item GPU Power Utilization with NVML
\end{itemize}

\subsection{Experimental Controls}
Assume that we are working on the simplest, most compute-optimized setting (i.e. FlashAttention, CUDA Graphs, etc.)
\begin{itemize}
    \item Dense data of static, fixed length
    \item Fixed Global Batch Size, Distributed over all GPUs
    \item Node Configuration (Constant for experiments for each cluster): Number of CPUs, Memory per Node
    \discuss{Consider fixing this to the minimal configuration common to all clusters -- e.g. control to fixed DRAM for all clusters}
    \item  Efficient Implementations: Flash Attention, Sparse Sequence Fast Paths, CUDA Graph serialization
    \item Deep Learning Frameworks: Megatron-LM, XLFormers
\end{itemize}

\subsection{Experimental Variables}
\paragraph{Hardware Acceleartors}
Reported numbers on compute and data speeds. We will empirically benchmark these numbers to build a practical cost model. 
\begin{table}[h!]
    \centering 
    \begin{tabular}{l|c|c|c|c}  \hline & \textbf{P100} & \textbf{V100} & \textbf{A100} & \textbf{H100} \\ \hline 
        {Tensor Core BF16 FLOPS}& 18.7 TFLOPS& 125 TFLOPS& 312 TFLOPS& approx 1000 TFLOPS \\ \hline 
        {GPU HBM} & 732 GB/s& 900 GB/s& 2 TB/s& 3.35 TB/s \\ \hline 
        {NVLink (GPU to GPU Comm.)}& NA& 300 GB/s& 600 GB/s& 900 GB/s \\ \hline 
        {PCIe (GPU to GPU Comm.)}& 32 GB/s& 32 GB/s& 64 GB/s& 128 GB/s \\ \hline 
    \end{tabular} \caption{Nvidia Reported GPU Specifications by Generation} 
\end{table}

        \begin{itemize}
            \item InfiniBand: $\sim400$ GB/s for sufficiently large data size with $\sim10\% $ slowdown scaling from 4 nodes to 256 nodes (32 to 256 GPUs)
            \item RocE-V2: $\sim 100$ GB/s from public resources
        \end{itemize}

 \paragraph{Training Configuration}
 \begin{itemize}
    \item Model Parameterizations:  1B, \textbf{7B}, 13B, 30B, 70B, 405B
    \item Data Precision: FP8 (Hopper Only), \textbf{BF16}, FP32
    \item Training Data Shapes:
    \begin{itemize}
        \item Sequence Length: 2k, \textbf{4k}, 8k, 32k
        \item Micro-Batch Size: 1, 2, 4, 8
    \end{itemize}
    \item Activation Checkpointing: All activations vs. selective layers for recomputation
\end{itemize}

\paragraph{Sharding and Parallelism Strategies}
    \begin{itemize}
        \item Distributed Data Parallel and Fully Sharded Data Parallel
        \item Model Parallel:
            Tensor, Sequence or Context, Pipeline Parallel
        \item DeepSpeed Offloading: Optimizer state, gradient, and parameter sharding
    \end{itemize}
\discuss{Q: What and when is data communicated or stored for each for each sharding strategy?}
\textbf{Bold} indicates the settings to be used for initial experimentation.

\section{Implementation Details}
For initial experiments, we use the internal XLFormers framework for training large language models on the V100 InfiniBand FAIR Cluster and the H100 CoreWeave cluster to investigate 

\discuss{Q: What is the experimental cross product we will be examining first?}
\discuss{Q:  We want a counter example to standard compute-bound assumptions. What setting is most likely to exhibit memory, data-bound behavior? }

\subsection{Compute Settings}
We consider settings representative of various standard computing regimes:
\begin{enumerate}
    \item 
\end{enumerate}

\subsection{Measurement Procedure}
\begin{enumerate}
    \item Distribute and synchronize model over $K_{//}$ GPUs 
    \item Warmup model with $K_{warmup}$ steps % I'd like to measure the variance here
    \item Synchronization Step; Measure elapsed time on the Rank 0 GPU for $K_{Sample}$ iterations
    \begin{enumerate}
        \item Question: Would there be a difference between measuring the total time for over multiple runs vs individual runs?
    \end{enumerate}

    \end{enumerate}

\section{Results and Analysis}
\begin{enumerate}
    \item Roofline Analysis of a given model configuration across hardware generations
\end{enumerate}



\section{Preliminaries and Initial Experiments}
\begin{enumerate}
    \item Setup an experimental harness for measurements of tokens per second and latency on V100 FAIR Cluster
    \item Create theoretical cost model
\end{enumerate}

\section{Additional Experiments and Extensions}
\begin{enumerate}
    \item Artificial network slowdowns on internode, multirail communications
\end{enumerate}


\section{Recommendations and Conclusions}
\begin{enumerate}
    \item Guidance on how to choose parallelism strategies
    \item Indicators, ranges over the dominant bottlenecks
\end{enumerate}


\section{Limitations}
In this work, we will primarily consider models based on the transformer architecture which is optimized, codesigned to achieve high levels of hardware utilization due to its heavy reliance on linear operations in both the MLP and Self-Attention layers.  In future work and as time allows, we will consider the distributed training performance of models for other modalities and architectures.

We consider settings representative of high-performance cluster computing settings-

\section{Timeline}
\begin{enumerate}
    \item June 24: Release Project Plan
\end{enumerate}

\section{Appendix}
Comparisons with existing work; Enumerating the differences in assumptions made
\begin{itemize}
    \item Aleph-Alpha Scaling   
    \item Megatron Scaling Analyses
    
    \item Mad Max
    \item DeepFlow
\end{itemize}

\paragraph{Ablation Experiments.}
\begin{itemize}
\item\textbf{Data. } Using real Llama-2 pretraining data as opposed to random, synthetic data
\item \textbf{Compute Optimizations. }Reduction in optimizations that improve compute utilization, disable: CUDA Graphs, Flash Attention, Fast Paths, FP32
\end{itemize}

\textbf{Additional Analyses}
\begin{itemize}
    \item Profiling of individual component FFN and Attention operations over common input and output shapes used in the model design; with additional search interpolating over intermediate shapes 
\end{itemize}

==> sections/B_framework.tex <==
\section{Empirical Scaling Laws for Distributed Training}
\label{sec:empirical_model}

\todo{change the word ``model'' to ``conceptual framework'' or ``methodology''}
\todo{Jared: Can we approximate blocking vs non-blocking }
\todo{This is where we include the toy diagram}

The empirical results from Sections \ref{sec:experimental_methodology} and \ref{sec:effects-of-scaling}\mostafa{I am not sure if you are referring to these 2 sections. Sec \ref{sec:experimental_methodology} does not have empirical results and Sec \ref{sec:effects-of-scaling} comes after not before this phrase.} motivate a clearer empirical model for the performance of model sharding that challenges both prior work and conventional wisdom around the applicability of sharding.

Recent work exploring the training dynamics of large neural networks has determined that there exists an optimal batch size for a given model parameterization or size, training compute budget (i.e. total FLOPs), and training data volume  \citep{kaplan2020scaling, porian2024resolving}. In practice, empirical research has arrived at stable recipes for training large models using fixed global batch sizes -- often relying on global batch sizes in the range of 1,000 to 2,000 tokens \citep{hoffmann2022empirical, hoffmann2022training, rae2021scaling}.\mostafa{Global batch size between 1,000 and 2,000 tokens is really small. I just checked Kaplan et al.  (OpenAI's scaling law paper), they had a context length of 1024 and global batch size of $2^{19}$.}

This model assumes the following setting: put a model $M$ with fixed, empirically motivated global batch size $\hat{b}$. We consider a distributed setup in which we have $n$ GPUs. We introduce two additional inputs: $b$, the batch size per-GPU, and $p$, the \textit{parallelism factor}, which can be described as the number of GPUs per model replica. A data-parallel setup has $p = 1$, whereas sharded setups feature $p > 1$.

It is clear by definition that $\hat{b} = \frac{n \cdot b}{p}$. Sharding increases the batch size per GPU for a fixed setup. We're interested in the following question: what are the conditions under which scaling from sharding level $p$ to $p'$ improves throughput? Such a change moves the batch size from $b$ per GPU to $b'$ where $b' = b \frac{p'}{p}$; the batch size per GPU scales by the change in parallelism.

We isolate two limiting factors to determine the total cost $c$ of moving to sharding level $p'$:
\begin{enumerate}
\item \textbf{Computation boundedness} --- many neural computation primitives (i.e. batched matrix multiplication) scale efficiently along the batch dimension; that is, increasing batch size by a factor $\frac{b'}{b}$ can be accomplished with a sublinear impact to computation time. We can introduce scale factor $s_{b'} = f(p, p')$ which denotes the factor change in computation time for new per-GPU batch size $s_{b'}$ for $p$ and $p'$. Given the effectiveness of batched primitives \citep{Thakkar_CUTLASS_2023}, it is not unusual that $s_{b'} < \frac{p'}{p}$ \citep{ModelBatchDomainParallelism}; matrix multiplication via feedforward layers accounts for the majority of computation time in large transformer-based models \citep{zhang2022opt}. We define $\frac{s_{b'}}{\frac{p'}{p}}$ as the computational return -- the factor cost of batch scaling relative to the factor increase in batch size.
    \begin{enumerate}
    \item \textbf{Relationship to model size} --- rather than sharding so as to change local batch size, we might also consider the effects of increasing model size, for example, by increasing the size of the hidden dimension. This might be considered a different case of scaling batched matrix multiplication, but scaling an intermediate dimension rather than an outer batch dimension.
    \item \textbf{Relationship to example context length} \todo{Complete this}
    \end{enumerate}
\item \textbf{Communication cost} --- the amount of exposed communication changes for a move to parallelism $p'$ is defined by a similar scaling factor which we denote $s_c = f(p, p')$. Typically, $s_c \geq \frac{p'}{p}$; communication cost scales at best linearly with sharding scale.
\end{enumerate}

Sharding to parallelism $p'$ improves performance \textit{if computational factor return exceeds additional exposed communication.} We can write the total sharding cost factor $c$ as the factor improvement in overall throughput for moving to parallelism $p'$ from $p$. We can model $c$ as follows:
\begin{equation}
\label{eq:shard_cost_model}
    c(p, p') = \frac{\frac{p'}{p}}{s_b} \cdot \left( \frac{\frac{p'}{p}}{s_c} - \ell(s_b, s_c) \right) \overset{?}{\lessgtr} 1
\end{equation}

where $\ell$ is a function which adjusts the impact of the scaled communication cost based on the amount by which new computation hides new or existing communication (i.e. $\ell$ is the amount of communication overlapped with computation). $c$ in Equation $\ref{eq:shard_cost_model}$ is a direct result of the product of computational and communication-related factor change; these jointly determine how performance changes with sharding. As such, we extend prior work \citep{Hsia2023MADMB, rashidi2021enabling, ardalani2024deepflow} that models exposed communication alone.

